Deceptive Planning for Resource Allocation

We consider a team of autonomous agents that navigate in an adversarial environment and aim to achieve a task by allocating their resources over a set of target locations. An adversary in the environment observes the autonomous team's behavior to infer their objective and responds against the team. In this setting, we propose strategies for controlling the density of the autonomous team so that they can deceive the adversary regarding their objective while achieving the desired final resource allocation. We first develop a prediction algorithm based on the principle of maximum entropy to express the team's behavior expected by the adversary. Then, by measuring the deceptiveness via Kullback-Leibler divergence, we devise convex optimization-based planning algorithms that deceive the adversary by either exaggerating the behavior towards a decoy allocation strategy or creating ambiguity regarding the final allocation strategy. A user study with $320$ participants demonstrates that the proposed algorithms are effective for deception and reveal the inherent biases of participants towards proximate goals.

==> beta_1.tex <==
\newcommand{\StaticObstacle}[2]{ \fill[] (#1+0,#2+0) rectangle  (#1+1,#2+1);}
\newcommand{\initialstate}[2]{ \fill[black!30!brown] (#1+0.1,#2+0.1) rectangle (#1+0.9,#2+0.9);}
\newcommand{\goalstate}[2]{ \fill[black!50!green] (#1+0.1,#2+0.1) rectangle (#1+0.9,#2+0.9);}
\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);

\fill[black!10!white] (0.05,0.05) rectangle (0.95,0.95);
\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);
\node[] at (0.5,0.5) {\Huge \textbf{S}};
\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/pred_true_beta_1}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};

\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);

\fill[black!10!white] (0.05,0.05) rectangle (0.95,0.95);
\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);
\node[] at (0.5,0.5) {\Huge \textbf{S}};
\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/pred_decoy_beta_1}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};
\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);


\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);

\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/exagg_beta_1}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};


\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);


\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);

\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/ambiguity_beta_1}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};


\end{tikzpicture}}
\end{subfigure}
\caption{Density distributions of the autonomous team. (Left) The distribution expected by the adversaries when the team aims to allocate their resources to achieve the final distribution $[0.5, 0.5, 0]$ over the goal states $[g_1, g_2, g_3]$. (Middle) The distribution expected by the adversaries when the team aims to allocate their resources to achieve the final distribution $[0, 0.5, 0.5]$ over the goal states $[g_1, g_2, g_3]$. (Right) The distribution generated under the proposed deceptive allocation strategy which achieves the true final distribution $[0.5, 0.5, 0]$ over the goal states $[g_1, g_2, g_3]$. The team exaggerates their behavior by pretending to achieve the decoy distribution $[0, 0.5, 0.5]$ along their paths.}
\label{tunable_figure}
\end{figure*}

==> beta_6.tex <==
\newcommand{\StaticObstacle}[2]{ \fill[] (#1+0,#2+0) rectangle  (#1+1,#2+1);}
\newcommand{\initialstate}[2]{ \fill[black!30!brown] (#1+0.1,#2+0.1) rectangle (#1+0.9,#2+0.9);}
\newcommand{\goalstate}[2]{ \fill[black!50!green] (#1+0.1,#2+0.1) rectangle (#1+0.9,#2+0.9);}
\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);

\fill[black!10!white] (0.05,0.05) rectangle (0.95,0.95);
\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);
\node[] at (0.5,0.5) {\Huge \textbf{S}};
\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/pred_true_beta_6}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};

\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);

\fill[black!10!white] (0.05,0.05) rectangle (0.95,0.95);
\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);
\node[] at (0.5,0.5) {\Huge \textbf{S}};
\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/pred_decoy_beta_6}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};
\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);


\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);

\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/exagg_beta_6}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};


\end{tikzpicture}}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
\centering
\scalebox{0.3}{
\begin{tikzpicture}
\draw[black,line width=0.4pt] (0,0) grid[step=1, very thin] (10,10);
\draw[black,line width=3pt] (0,0) rectangle (10,10);


\fill[black!10!white] (0.05,9.05) rectangle (0.95,9.95);
\fill[black!10!white] (4.05,9.05) rectangle (4.95,9.95);
\fill[black!10!white] (9.05,9.05) rectangle (9.95,9.95);

\node[] at (0.5,9.5) {\Huge $\boldsymbol{g_1}$};
\node[] at (4.5,9.5) {\Huge $\boldsymbol{g_2}$};
\node[] at (9.5,9.5) {\Huge $\boldsymbol{g_3}$};

\StaticObstacle{1}{2}
\StaticObstacle{2}{2}
\StaticObstacle{1}{3}
\StaticObstacle{2}{3}

\StaticObstacle{6}{3}
\StaticObstacle{7}{3}
\StaticObstacle{6}{4}
\StaticObstacle{7}{4}

\StaticObstacle{3}{6}
\StaticObstacle{4}{6}
\StaticObstacle{5}{6}
\StaticObstacle{3}{7}
\StaticObstacle{4}{7}
\StaticObstacle{5}{7}

\input{tikz_grid_values/ambiguity_beta_6}

\fill[black!10!white] (2.05,0.05) rectangle (2.95,0.95);
\node[] at (2.5,0.5) {\Huge \textbf{S}};


\end{tikzpicture}}
\end{subfigure}
\caption{Density distributions of the autonomous team. (Left) The distribution expected by the adversaries when the team aims to allocate their resources to achieve the final distribution $[0.5, 0.5, 0]$ over the goal states $[g_1, g_2, g_3]$. (Middle) The distribution expected by the adversaries when the team aims to allocate their resources to achieve the final distribution $[0, 0.5, 0.5]$ over the goal states $[g_1, g_2, g_3]$. (Right) The distribution generated under the proposed deceptive allocation strategy which achieves the true final distribution $[0.5, 0.5, 0]$ over the goal states $[g_1, g_2, g_3]$. The team exaggerates their behavior by pretending to achieve the decoy distribution $[0, 0.5, 0.5]$ along their paths.}
\label{tunable_figure}
\end{figure*}

==> idle.tex <==
\subsection{Resource allocation games}
We formally define the resource allocation game as a zero-sum game between two teams, namely, Team 1 and Team 2. In this game, each team has an allocation strategy that describes the final spatial distribution of their available resources in the environment. 

Let $\mathcal{G}$$:=$$\{g_1,g_2,\ldots,g_k\}$$\subset$$\mathcal{S}$ be a set of \textit{absorbing goal states} in the environment. Moreover, let $U$$\in$$\mathbb{R}^{k \times k}$ be a utility matrix where $U_{i,j}$ expresses the utility gained by Team 1 and lost by Team 2 when they allocate all their resources to $g_i$ and $g_j$, respectively. 

In resource allocation games, the teams allocate their resources to optimize their utility. Formally, let $\sigma_1$$:$$\mathcal{G}$$\rightarrow$$[0,1]$ be the allocation strategy for Team 1 such that $\sum_{g_i\in \mathcal{G}}\sigma_1(g_i)$$=$$1$. Similarly, let $\sigma_2$$:$$\mathcal{G}$$\rightarrow$$[0,1]$ be the allocation strategy for Team 2 such that $\sum_{g_i\in \mathcal{G}}\sigma_2(g_i)$$=$$1$. For notational convenience, we denote the vector representation of the allocation strategies as $\boldsymbol{\sigma}_1, \boldsymbol{\sigma}_2$$\in$$[0,1]^{k}$. Finally, we denote the set of all available strategies for Team 1 and Team 2 by $\Sigma_1$ and $\Sigma_2$, respectively.

We formally define the resource allocation game as the following zero-sum game
\begin{align}
    \max_{\boldsymbol{\sigma}_1\in \Sigma_1} \min_{\boldsymbol{\sigma}_2\in \Sigma_2} \boldsymbol{\sigma}_1^TU\boldsymbol{\sigma}_2.
\end{align}

{\setlength{\parindent}{0cm}
\noindent \begin{definition} 
For a resource allocation game with the utility matrix $U$$\in$$\mathbb{R}^{k \times k}$, a pair $(\boldsymbol{\sigma}_1^{\star}, \boldsymbol{\sigma}_2^{\star})$$\in$$\Sigma_1$$\times$$\Sigma_2$ of strategies are said to be \textit{equilibrium strategies} if they satisfy
\(
 \boldsymbol{\sigma}_1^TU\boldsymbol{\sigma}_2^{\star} \leq \boldsymbol{\sigma}_1^{{\star}  T}U\boldsymbol{\sigma}_2^{\star} \leq \boldsymbol{\sigma}_1^{\star T}U\boldsymbol{\sigma}_2
\)
for all $\boldsymbol{\sigma}_1\in\Sigma_1$ and $\boldsymbol{\sigma}_2\in\Sigma_2$
\end{definition}}

Equilibrium strategies for the resource allocation game express the \textit{final} spatial densities of the resources in the environment. For example, if $\sigma_1^{\star}(g_1)$$=$$\sigma_1^{\star}(g_2)$$=$$1/2$, it means that Team 1 aims to deploy half of its resources to the goal state $g_1$ and the other half to the goal state $g_2$ by starting the process from the initial spatial distribution $\alpha$. We note that, for a given utility matrix, equilibrium strategies can be efficiently computed via linear programming \cite{bacsar1998dynamic}.



We consider two potential utility matrices, i.e., $\mathcal{U}$$=$$\{U_1, U_2\}$, where
\begin{align*}
    U_1 = \begin{bmatrix} 0 & 0 & 6 \\
    0 & 2 & 0 \\
    -1 & 0 & 0 
    \end{bmatrix},\ \  \text{and} \ \ 
    U_2 = \begin{bmatrix} 0 & 0 & -1 \\
    0 & 2 & 0 \\
    6 & 0 & 0 
    \end{bmatrix}.
\end{align*}
The interpretation of the utility matrices are as follows. For the first utility matrix $U_1$, the goal state $g_1$ is the most critical location. Specifically, if the team allocate all their resources to $g_3$ while the adversaries allocate their resources to $g_1$, the team incurs a negative payoff. On the other hand, if the team allocates all their resources to $g_1$ while the adversaries occupy $g_3$ with all their resources, then the team gains a utility of $6$. Furthermore, if both teams allocate their resources to $g_2$ at the same time, then Team 1 gains a payoff of $2$ since it is in their benefit to engage in a competition in this state. For the second utility matrix $U_2$, we have the same interpretation with the goal state $g_3$ being the most critical location.

We compute a pair of equilibrium strategies for both utility matrices by solving the corresponding linear programs. A set of equilibrium strategies are given as $(\boldsymbol{\sigma}_{1,U^1}^{\star}, \boldsymbol{\sigma}_{2,U^1}^{\star})$$=$$([0.5, 0.5, 0], [1, 0, 0])$ and $(\boldsymbol{\sigma}_{1,U^2}^{\star}, \boldsymbol{\sigma}_{2,U^2}^{\star})$$=$$([0, 0.5, 0.5], [0, 0, 1])$.




\draw[draw=black, fill = lightgray, opacity = 0.4, rounded corners](-7.5,1.75) rectangle ++(6,1.75);

\node[align = center] at (-4.6,3.15) {\Large Potential goal distributions};

\node[text width = 1.5 cm,align = center] at (-5.2,2.55) {\large $\mathcal{U}$$=$$\{\boldsymbol{\sigma}_{1},\ldots,\boldsymbol{\sigma}_{N}\}$};

\draw[->, thick] (-1.5,2.75) -- (2.5,2.75);


\draw[->, thick] (7.5,2.75) -- (11,2.75);
\node[text width = 4 cm,align = center] at (9.2,3.8) {\large Predicted policies};
\node[text width = 4 cm,align = center] at (9.2,3.2) {\large $\{\overline{\pi}_i, \ i$$\in$$[N]\}$};


